Enhancing Manufacturing Quality Prediction Models through the Integration of Explainability Methods

This research presents a method that utilizes explainability techniques to amplify the performance of machine learning (ML) models in forecasting the quality of milling processes, as demonstrated in this paper through a manufacturing use case. The methodology entails the initial training of ML models, followed by a fine-tuning phase where irrelevant features identified through explainability methods are eliminated. This procedural refinement results in performance enhancements, paving the way for potential reductions in manufacturing costs and a better understanding of the trained ML models. This study highlights the usefulness of explainability techniques in both explaining and optimizing predictive models in the manufacturing realm.

==> old.tex <==

\subsubsection{Analyzing Prediction Effectiveness at Various Data Collection Intervals}
In manufacturing sectors, the ability to accurately predict the final quality of a workpiece during its processing stage is of paramount significance. This predictive insight allows for timely interventions and adjustments, potentially saving time and resources. This experiment aims to scrutinize the prediction effectiveness at different stages of data collection during the workpiece processing cycle.
This investigation considers a dynamic process wherein a workpiece undergoes a manufacturing stage. 
The critical aspect we intend to scrutinize is how prediction accuracy varies with the proportion of data accumulated during the manufacturing phase. 

\paragraph{Setup.} To achieve the previously mentioned objective, we delineate several intervals, such as 10\%, 20\%, and 30\%, representing the fractions of the total processing time data.


\paragraph{Execution.} We then employ our trained ML models to assess the quality of the final piece based on data collected up until each of these intervals. We compare these predictions with the final quality measured at 100\% of the data collection time to evaluate the efficacy of predictions made at earlier stages.
In this experiment, we focused on one ML model, the decision tree regression model, to illustrate the main findings.
The results for the other models can be found in the Appendix.

\paragraph{Findings.} Based on the experiment (see Figure~\ref{fig:partial_predictions}), we observed that achieving the same quality prediction results with fewer data is possible than having 100\% of the data available.
This insight suggests that earlier interventions might be feasible to improve the workpiece quality further.
Furthermore, we noticed that the minimum amount of data needed to achieve reliable predictions fluctuated for varying quality measurements. 

This experiment substantiates the possibility of making reliable predictions about the final quality of a workpiece during different phases of its processing cycle.
It underscores the potential for optimizing manufacturing processes through timely interventions, enhancing overall efficiency and product quality.
\begin{figure*}[]
    \centering
    \includegraphics[width=15.5cm]{errors_10000_decision tree.png}
    \caption{CASE STUDY I  mean absolute error for quality predictions given a specific percentage of the time series data (to simulate the prediction process during workpiece processing).}
    \label{fig:partial_predictions}
\end{figure*}

